Semi-Automated Modular Formal Verification of Critical Software: Liveness and Completeness Thresholds

In this dissertation we describe two contributions to the state of the art in reasoning about liveness and safety, respectively. Programs for multiprocessor machines commonly perform busy waiting for synchronization. We propose the first separation logic for modularly verifying termination of such programs under fair scheduling. Our logic requires the proof author to associate a ghost signal with each busy-waiting loop and allows such loops to iterate while their corresponding signal $s$ is not set. The proof author further has to define a well-founded order on signals and to prove that if the looping thread holds an obligation to set a signal $s'$, then $s'$ is ordered above $s$. By using conventional shared state invariants to associate the state of ghost signals with the state of data structures, programs busy-waiting for arbitrary conditions over arbitrary data structures can be verified. Moreover, we present the first study of completeness thresholds for bounded memory safety proofs. Specifically, we consider heap-manipulating programs that iterate over arrays without allocating or freeing memory. In this setting, we present the first notion of completeness thresholds for program verification which reduce unbounded memory safety proofs to bounded ones. Furthermore, we demonstrate that we can characterise completeness thresholds for simple classes of array traversing programs. Finally, we suggest avenues of research to scale this technique theoretically, i.e., to larger classes of programs (heap manipulation, tree-like data structures), and practically by highlighting automation opportunities.

==> chapters/abstract/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:04 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: abstract.pdf
abstract.pdf: 
	( cd "$(MAINDIR)" && make chapters/abstract/$@ )

.PHONY: bare abstract_bare.pdf
bare: abstract_bare.pdf
abstract_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/abstract/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/abstract/abstract.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard abstract*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) abstract.pdf abstract_bare.pdf

s:
	@echo gvim abstract.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/abstract/abstract.tex <==
% !TeX root = ../../thesis.tex
\chapter{Abstract}                                 \label{ch:abstract}

In this dissertation we describe two contributions to the state of the art in reasoning about liveness and safety, respectively.

Programs for multiprocessor machines commonly perform busy waiting for synchronization. 
We propose the first separation logic for modularly verifying termination of such programs under fair scheduling. 
Our logic requires the proof author to associate a ghost signal with each busy-waiting loop and allows such loops to iterate while their corresponding signal~$s$ is not set. 
The proof author further has to define a well-founded order on signals and to prove that if the looping thread holds an obligation to set a signal $s'$, then $s'$ is ordered above $s$. 
By using conventional shared state invariants to associate the state of ghost signals with the state of data structures, programs busy-waiting for arbitrary conditions over arbitrary data structures can be verified.

Moreover, we present the first study of completeness thresholds for bounded memory safety proofs. 
Specifically, we consider heap-manipulating programs that iterate over arrays without allocating or freeing memory. 
In this setting, we present the first notion of completeness thresholds for program verification which reduce unbounded memory safety proofs to bounded ones. 
Furthermore, we demonstrate that we can characterise completeness thresholds for simple classes of array traversing programs. 
Finally, we suggest avenues of research to scale this technique theoretically, i.e., to larger classes of programs (heap manipulation, tree-like data structures), and practically by highlighting automation opportunities.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/abstractnl/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:05 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: abstractnl.pdf
abstractnl.pdf: 
	( cd "$(MAINDIR)" && make chapters/abstractnl/$@ )

.PHONY: bare abstractnl_bare.pdf
bare: abstractnl_bare.pdf
abstractnl_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/abstractnl/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/abstractnl/abstractnl.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard abstractnl*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) abstractnl.pdf abstractnl_bare.pdf

s:
	@echo gvim abstractnl.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/abstractnl/abstractnl.tex <==
% !TeX root = ../../thesis.tex
\chapter{Beknopte samenvatting}

In dit proefschrift beschrijven we twee bijdragen aan de state-of-the-art in redeneren over respectievelijk liveness en safety.

Programma's voor multiprocessor machines maken gebruik van busy waiting voor synchronisatie.
Wij stellen de eerste separation logic voor om modulair de beëindiging van zulke programma's onder fair scheduling te verifiëren.
Onze logica vereist dat de auteur van het bewijs een ghost signal toekent aan elke busy waiting lus. 
Deze lussen mogen itereren zolang hun corresponderende signaal $s$ niet is ingesteld.
De auteur van het bewijs moet daarnaast een welgefundeerde orderelatie op signalen definiëren, en moet daarbovenop bewijzen dat als de looping thread een obligatie van een signal $s'$ bezit, dat $s'$ groter is dan $s$.
Door klassieke gedeelde toestandsinvarianten te gebruiken om de toestand van ghost signals te associëren met de toestand van datastructuren, kunnen programma's met busy waiting geverifiëerd worden, voor arbitraire condities over arbitraire datastructuren.

Daarnast presenteren we de eerste studie naar completeness thresholds voor bounded memory safety bewijzen. 
Specifiek beschouwen we heap-manipulerende programma's die itereren over arrays zonder het toekennen of vrijgeven van geheugen.
In deze context presenteren we de eerste notie van completeness thresholds voor programmaverificatie die unbounded memory safety bewijzen reduceren tot bounded bewijzen. 
Tevens laten we zien dat we completeness thresholds kunnen karakteriseren voor eenvoudige klassen van programma's die arrays doorlopen. 
Tot slot suggereren we theoretische onderzoekspistes voor grotere klassen van programma's (heapmanipulatie, boomachtige datastructuren), en praktische mogelijkheden voor bewijsautomatisatie.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/conclusion-template-backup/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:05 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: conclusion-template-backup.pdf
conclusion-template-backup.pdf: 
	( cd "$(MAINDIR)" && make chapters/conclusion-template-backup/$@ )

.PHONY: bare conclusion-template-backup_bare.pdf
bare: conclusion-template-backup_bare.pdf
conclusion-template-backup_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/conclusion-template-backup/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/conclusion-template-backup/conclusion-template-backup.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard conclusion-template-backup*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) conclusion-template-backup.pdf conclusion-template-backup_bare.pdf

s:
	@echo gvim conclusion-template-backup.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/conclusion-template-backup/conclusion.tex <==
% !TeX root = ../../thesis.tex
\chapter{Conclusion (Template)}\label{ch:conclusion}

\ldots

\instructionsconclusions

\TodoTextNote{Get rid of template's dummy conclusion and write one that mentions TadaLive.}


\TodoTextNote{
	Discuss:
	\begin{itemize}
		\item TadaLive
		\item Peter Müller's work on verifying absence of blocking
		\item Marieke Huismann's work on verifying termination of programs using await statements:
	\end{itemize}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/conclusion/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:05 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: conclusion.pdf
conclusion.pdf: 
	( cd "$(MAINDIR)" && make chapters/conclusion/$@ )

.PHONY: bare conclusion_bare.pdf
bare: conclusion_bare.pdf
conclusion_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/conclusion/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/conclusion/conclusion.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard conclusion*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) conclusion.pdf conclusion_bare.pdf

s:
	@echo gvim conclusion.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/conclusion/conclusion.tex <==
% !TeX root = ../../thesis.tex
\chapter{Conclusion and Future Work}\label{ch:conclusion}

In this thesis we described two contributions to the state of the art in reasoning about liveness and safety, respectively.
The following sections~\ref{sec:conclusion:liveness} and \ref{sec:conclusion:ct} reflect on the contributions we presented in \S~\ref{ch:paper-2-ghostSignals} and \S~\ref{ch:paper-3-ct4ms}, respectively, and outline directions for future work.

\section{Liveness Verification}\label{sec:conclusion:liveness}

\paragraph{Ghost Signals}
In \S~\ref{ch:paper-2-ghostSignals} we presented the first separation logic to modularly verify termination of concurrent programs involving busy waiting.
%Separation logic is a safety logic.
%That is, in its standard form it only allows us to prove safety and partial correctness properties.
Standard separation logic only allows us to prove safety and partial correctness properties.
Safety properties are much better understood and easier to verify than liveness properties.
This is particularly true due the wealth of Hoare-style~\cite{Hoare1968HoareLogic} logics that have been developed for safety verification
\cite{OHearn2012APO,
	Owicki1976VerifyingPropiertiesGhostVariables,
	Xu1997RelyGuarentee,
	VafeiadisCSLSound,
	Vafeiadis2007RGSep,
	Jung2018IrisGroundUp,
	Lundberg2020HoareStyleLogic}
.
% Overview of Hoare-style logic evolution:
% https://johnwickerson.github.io/talks/rely_guarantee.pdf
%
Hoare triples  \hoareTriple{A}{c}{B} like the ones used in separation logic allow us to reason locally and intuitively.
The logic we presented in \S~\ref{ch:paper-2-ghostSignals} inherits these advantages by extending separation logic.
Moreover, extending a standard separation logic made it easy to implement our approach in VeriFast, a separation logic based program verifier for C.


Our approach to verifying termination is to reduce it to safety.
We do this by introducing a new type of ghost resource called \emph{ghost signal}.
These signals only exist on the proof level and each is tied to an event a thread might wait for.
Creating a ghost signal also spawns an obligation -- another ghost resource -- to perform said event.
Our logic ensures that no thread terminates with undischarged obligations.
It also takes care to rule out cyclic wait dependencies that could lead to non-terminating wait loops.
%Note that the latter two are safety properties.
Since the latter two are safety properties, we indeed reduced liveness to safety.

Busy waiting verification is an active area of research. 
In the remainder of this section, we briefly discuss TaDA Live, the main new development in this area since our work appeared.
We also briefly discuss an ongoing project of our research group continuing our ghost signal work.
Afterwards, we briefly sketch another active research area: Reasoning about liveness in step-indexed logics.

\paragraph{TaDA Live}
\citeauthor{DOsualdo2021TadaLive}
propose TaDA Live~\cite{DOsualdo2021TadaLive},
a separation logic to verify termination of programs that involve blocking, fine-grained concurrency, e.g., busy waiting for a heap cell to be set.
The paper was submitted in parallel to our ghost signal paper (cf.~\S~\ref{ch:paper-2-ghostSignals})
and published shortly after it.
Both approaches share similarities such as the use of obligations and levels (or layers in TaDA Live terms) to reason about dependencies.
Those aside, their logic differs widely from ours.
TaDA Live offers a notion of liveness invariants $\displaystyle\square\lozenge P$, expressed in terms of subjective obligations and guards~\cite{Dodds2009DenyGuaranteeReasoning}.
Their obligations are subjective in the sense introduced by \citeauthor{Ley-Wild2013SubjectiveAuxiliaryState}~\cite{Ley-Wild2013SubjectiveAuxiliaryState}.
That is, they support two different perspectives: Local and environment.
This makes knowledge about the environment duplicable and a first class citizen in TaDA Live.
(The term \emph{duplicable} should not be confused with Iris' notion of duplicable assertions~\cite{Jung2018IrisGroundUp}.
In Iris, duplicable assertions are assertions that remain true forever.
This is not the case here, since in TaDA~Live duplicable assertions are not necessarily stable.)

TaDA Live offers a notion of abstract atomic specifications to specify blocking behaviour.
This allows them to assign reusable and provable specifications to, e.g., spin and CLH locks.
Moreover, TaDA Live's liveness invariants offer a great deal of flexibility and control to the client over when subjective obligations are spawned and discharged.
In general, the client is responsible for proving that it enforces the liveness assumptions required by the lock specifications.
%This allows them to verify programs where a lock is acquired but never released as long as no other thread tries to acquire it.
This allows them to verify programs where a lock is acquired in one thread but released in another one.
Our ghost signal work does not concern the question of how to construct optimally abstract yet expressive specifications for busy-waiting modules. 


The expressiveness that TaDA Live offers comes at the price of a proof system that is significantly more complex than ours.
Hence, it is also harder to mechanize.
In particular, TaDA Live is an unstable separation logic.
%That is, assertions are unstable in the sense that they can be invalidated by other threads.
That is, not all assertions are stable in the sense that assertions can generally be invalidated by other threads.
%
% Meanwhile, Hoare triples in TaDA Live require stability.
% Every time we want to use one we have to prove that every program step preserves stability.
% > According to Bart this description is incorrect.
%
% TaDA Live paper, sec. 2.1, p. 14
% "The Hoare pre-/post-conditions describe stable resources that are owned locally by C and can be updated non-atomically."
Meanwhile, assertions used as pre- or postconditions in Hoare triples require stability 
since they describe locally owned resources.
That is, if a relevant shared region protocol permits the environment to take a transition, then we have to prove that this transition does not invalidate the assertion.
%
%
In contrast, we implemented our ghost signals and our CLH lock case study in VeriFast~\cite{Jacobs2011Verifast}.
Since VeriFast is a stable separation logic, it is difficult or impossible to use it to implement TaDA Live.
For the same reason, it is hard or impossible to implement TaDA Live in the popular mechanised separation logic Iris~\cite{Jung2018IrisGroundUp}.
There is, however, a proof checker called Voila~\cite{Wolf2023_JournalFMSD_TaDACheckerVoila, Wolf2021_FM_TaDACheckerVoila} for TaDA~\cite{Pinto2014TaDA} a predecessor of TaDA Live.



%\revRemark[Bart's feedback]{
%	"Every time we want to use one we have to prove that every program step preserves stability.": I couldn't figure this sentence out. Note that TaDA Live is not like the interference-freedom Owicki-Gries approach where you have to check, for every assertion in the proof outline of one thread, that they are preserved by the commands of parallel threads. Instead, in TaDA Live, you have to prove, for each assertion, that it is preserved by shared region transitions not ruled out by local ownership of guards (roughly speaking).
%}

Since the publication of our ghost signal paper, we focused on different research areas.
Meanwhile, our research group, specifically \citet{Fasse2023IrisWS_modularSpecs}, continues this line of work.

TaDA Live also supports specifying the abstract blocking behaviour of spin and CLH lock~\cite{herlihy-multiprocessor} implementations as well as a flexible handling of obligations.
%This escapes the scope of our ghost signal logic and we consider it future work.
%Instead we axiomatised primitive acquire and release operations.
%\citeauthor{Fasse2023IrisWS_modularSpecs} are continuing our research~\cite{Fasse2023IrisWS_modularSpecs}.
The ongoing work of \citet{Fasse2023IrisWS_modularSpecs} extends our ghost signal logic to support more flexible, modular lock specifications for various lock implementations such as spin, CLH, ticket~\cite{Mellor1991TicketLock} and cohort~\cite{Dice2012CohortLock, Dice2015CohortLock} locks.
In order to verify the latter one, they need to treat the creation of obligations more flexibly than it is currently the case in our ghost signal work.
They achieve this flexibility by letting the client create the obligations instead of the module.
In the example lock specifications we developed, every acquire call spawns an obligation to release the lock.
Since we do not allow threads to pass obligations to arbitrary other threads, this means that we force the acquiring thread to eventually release it.
In a cohort lock, however, an acquired lock can be passed on to another thread within the same cohort without releasing it.
Our logic does not support these \emph{hand-offs}.
By passing on the lock, the original owner loses their chance to discharge their release obligation.
Moreover, \citeauthor{Fasse2023IrisWS_modularSpecs} are working on mechanising their logic in Iris.

\paragraph{Liveness and Step-Indexed Logics}
Reasoning about liveness in step-indexed logics is an active research topic~\cite{Tassarotti2017ConcurrentTerminationRefinement, Spies2021TransfiniteIris, Timany2024Trillium}.
The main challenge is to overcome the restriction that by default, step-indexed logics only allow reasoning about finite execution prefixes.

\citet{Tassarotti2017ConcurrentTerminationRefinement} focus on verifying liveness in concurrent settings that only have bounded non-determinism (i.e. languages where each state has only finitely many successors).
This restriction allows them to extend Iris to reason about fair termination-preserving refinement.
\citet{Spies2021TransfiniteIris} propose Transfinite Iris which uses ordinals instead of natural numbers as step indices.
Using these transfinite step indices instead of finite ones allows them to reason about termination and termination-preserving refinement in non-concurrent programs.
\citet{Timany2024Trillium} propose Trillium, a separation logic framework to prove intensional refinement relations between a program and an abstract model given as transition system.
In particular, they consider liveness-preserving refinements concerning concurrent programs under fair scheduling.


 
 
 
\section{Completeness Thresholds}\label{sec:conclusion:ct}


%\paragraph{Completeness Thresholds}
In \S~\ref{ch:paper-3-ct4ms} we presented the first notion of completeness thresholds (CT) for software verification, which allows to obtain unbounded guarantees from bounded proofs.
To be precise, we study CTs for memory safety proofs of array traversing programs.
Bounded verification approaches like bounded model checking (BMC) offer a high degree of automation and convenience.
Yet this comes at the expense of soundness, since they only explore a finite number of finite execution prefixes.
Bounded model checkers require the user to set two types of bounds upfront:
(i)~A bound for input data and
(ii)~a depth bound limiting the size of the explored execution prefixes (or alternatively distinct depth bounds for each loop and recursive function call).
In this work, we focus on bounding input data.
In practice, coming up with meaningful bounds is very difficult and requires the user to take both the target program into account and also the class of errors they want to find.

\myComment{
	\TodoTextNote[Bart's feedback: Delete]{
		\paragraph{Intuition Behind CTs}
		Consider a program with an input variable \varVar of domain~\domVar.
		%
		%A CT for \varVar is a subdomain $\ctVar \subseteq \domVar$ big enough to ensure that a bounded proof restricted to \ctVar yields the guarantees as one fully exploring \domVar.
		%
		A CT for \varVar is a subdomain $\ctVar \subseteq \domVar$ big enough to ensure that a proof restricted to \ctVar remains sound regardless of the bounding.
		A bounded proof is unsound if it misses bugs, which is the case if the domain restriction excludes inputs that are necessary to reach errors.
		Hence, intuitively speaking, a subdomain $\ctVar \subseteq \domVar$ is a CT if it covers all elements required to reach potential memory safety errors.
		If we know that this is the case, we know that a successful bounded proof refuted all potential errors that might arise during execution.
		Hence, we can conclude that the program is indeed memory safe.
	}
}

\paragraph{Extracting CTs from VCs}
CTs are a concept originally developed in the context of model checking finite state transition systems~\cite{Biere1999SymbolicMC, Clarke2004CompletenessAC}.
In this context CTs are natural numbers that bound the length of path prefixes a model checker needs to explore to produce a sound proof.
The finite nature of these transition systems allows for the characterisation of CTs in terms of key properties of the transition system.
Programs processing arbitrarily large data structures, however, correspond to infinite transition systems where said key properties are often infinite.
Naively applying existing approaches would hence lead to infinite and thus unusable CTs.
Instead we study a program's verification condition~(VC).
The VC reflects all potential memory errors that might arise during the program execution.
Most importantly, it shows how different classes of concrete inputs influence the correctness of the program.
In our work, we show that we can extract a CT \ctVar for a variable \varVar by extracting a validity preserving subdomain $Y \subseteq \domVar$ from a VC.
We prove that $Y$ is validity preserving by restricting \varVar in the VC to $Y$ and then rewriting the VC until we eliminated~\varVar.
If this succeeds, the concrete choice of $\varVar \in Y$ does not affect whether or not a memory error occurs in our program.
That is, we can collapse the entire subdomain $Y$ to an arbitrary representative $y \in Y$.
Hence, we found our CT $\ctVar = \domVar \setminus Y \cup \setOf{y}$.


\paragraph{Increasing Trust in BMC}
The state space explosion problem and resource constraints make it often only practical to explore small bounds.
%BMC proofs can often only explore small bounds due to the state space explosion problem.
Especially traversing over data structures drives up the computational costs.
Obtaining small CTs for the size of the traversed structure does not only allow us to obtain unbounded guarantees with respect to one dimension of the proof.
In many cases it will also allow us to reduce the explored size bound and thereby significantly speed up the proof.
We can then reinvest the freed up computation resources into checking more critical bounds.
That is, we can increase another bound while maintaining the proof's overall performance.
Hence, ultimately we obtain a bounded proof we can trust significantly more.


As this is an ongoing project, there are several angles that we are going to study further.

\paragraph{Limitations of CTs}
In general, VCs over-approximate a program's correctness behaviour.
That is, it is possible that the VC does not hold, even though the program is correct.
We have to be careful about this when relating CTs that we extracted from a VC back to the original program.
We are currently investigating this relationship and found that CTs for a variable~\varVar extracted from a VC hold for the program iff the VC does not over-approximate the influence of~\varVar on the correctness of the program.
Note that this is a significantly weaker restriction than requiring that the VC as a whole does not over-approximate.
In appendix~\S~\ref{ch:appendix-paper-3-ct4ms} we formalise this relationship and call such VCs \emph{precise}~in~\varVar~(cf.~Def.~\ref{ct4msTR:appendix:def:preciseVerificationCondition}).
Moreover, we prove a soundness~theorem~(cf.~Theo.~\ref{ct4msTR:appendix:soundness}) stating that precision is a sufficiently strong requirement to ensure soundness of any extracted CT with respect to the original program specification.

Note that this applies to the array traversal pattern and its VC studied in~\S~\ref{ch:paper-3-ct4ms}.
Loops are a common cause for over-approximations in VCs.
Meanwhile, iteration over data structures is a common cause for exponential blow ups in model checking.
Therefore, we are going to focus on common traversal patterns for inductive data structures.
We are going to study whether their VCs over-approximate with respect to the size of the traversed data structures.
In case we find that they do not, we plan to manually compute CTs for the most common patterns.
Model checkers could then automatically search for these patterns and directly apply our CTs to speed up the model checking process.



\paragraph{Scaling}
%The array traversal pattern that we studied in \S~\ref{ch:paper-3-ct4ms} is quite simple.
Ultimately, we want to extract CTs for realistic programs that are much more complex than the array traversal pattern studied in \S~\ref{ch:paper-3-ct4ms}.
To achieve this, we are going to look into several different directions:

(i)~We are going to study the combinatorial properties of memory safety CTs.
As already sketched in the outlook of \S~\ref{ch:paper-3-ct4ms}, we can exploit the structure of a program when extracting CTs.
We are going to investigate how control structures allow us to extract a CT by combining CTs from their respective sub-ASTs.
Once we know sufficiently many CT combinators, we will be a big step closer to extracting CTs from realistic programs.

(ii)~Consider a program that traverses an array, reads elements and uses the read values for some further computation~$f$ not involving the array nor its size~\sizeVar.
Intuitively, $f$ should not affect the CT for~\sizeVar.
Yet, VCs tend to get very complex very fast.
Hence, proving that we can ignore the sub-VC corresponding to $f$ proves tricky on the VC level.
Meanwhile, program slicing~\cite{Weiser84ProgramSlicing} is an established technique that allows us to do exactly that: 
Slicing off the parts of the program not affected by \sizeVar.
We are going to look into this.
It seems promising that (i)~and~(ii) together will allow us to compute array-size CTs for realistic programs traversing arrays.

(iii)~We are also going to investigate CTs for programs traversing inductive data structures besides arrays, e.g., lists and trees.
The mechanism of extracting a CT remains the same regardless of the data structure.
The VC, however, and also the traversal patterns we need to study grow in complexity with the traversed structure.
We are confident that extending our results to lists will be straight-forward.
Though, we expect it to be more difficult to do the same for tree structures.
Mainly because of the complexity of common traversal patterns like breadth-first-search.



\paragraph{Case Study}
Once we are able to extract CTs for realistic programs, we plan to empirically evaluate their impact on the runtime of industrial-grade BMC proofs.
Our evaluation target will be FreeRTOS's TCP/IP stack~\cite{repo_FreeRTOS_tcp}.
FreeRTOS~\cite{website_FreeRTOS} is an open source, real-time operating system used by many commercial IoT vendors.
The FreeRTOS team heavily relies on CBMC -- an industrial-strength, open source bounded model checker -- to ensure the correctness of their system.
In particular, the repository of their TCP stack contains many CBMC proofs for functions traversing over TCP buffer arrays.
We plan to select a number of these functions, which we then manually transcribe to the WHILE language we study in our CT work.
Once we extracted CTs from those transcribed programs, we are going to apply them to the existing CBMC proofs and measure the speed up.
We are going to run each proof with two sets of bounds:
Once with its original bounds and once with minimal bounds according to the extracted CTs.
The runtime difference, will then be the speed up we can attribute to our CTs.

We are aware that CTs extracted from transcribed programs are not a perfect fit for the original C programs.
There's always a risk that the transcription misses some intricacies of C semantics.
However, we are confident that these experiments are sufficiently precise to convey insights into the magnitude of speed up CTs allow for.




\paragraph{Generalise CTs}
At last, we are currently working on generalising CTs to arbitrary correctness properties.
We found that this is straight-forward for the theoretical foundations of our work, i.e., the definition of CTs and all theorems presented in \S~\ref{ch:paper-3-ct4ms} and appendix~\S~\ref{ch:appendix-paper-3-ct4ms}.

In appendix~\S~\ref{ch:appendix-genCTsTR} we present a generalised CT theory that considers an abstract notion of program correctness.
Thereby, it covers both safety and liveness properties such as memory safety and termination, but also more complex functional correctness properties.
In particular, it subsumes the memory safety CT~theory presented in appendix~\S~\ref{ch:appendix-paper-3-ct4ms}.
We present a generalised notion of precision (cf.~Def.~\ref{genCTsTR:appendix:def:preciseVerificationCondition}) and a soundness theorem (cf.~Theo~\ref{genCTsTR:appendix:theo:precision}) for the generalised theory. 
The latter states that (analogous to the special case, cf.~Theo.~\ref{ct4msTR:appendix:soundness}) precision is a sufficiently strong requirement to ensure soundness of any extracted CT with respect to the original program specification.
Moreover, we show that -- following the intuition behind CTs -- CTs are subdomains that cover error equivalence classes (cf.~Theo.~\ref{genCTsTR:appendix:theo:ErrorCoverCT}).
This justifies extracting CTs by factoring out potential error equivalence classes.

Most of the time, it is sufficient to treat correctness as an arbitrary predicate.
The same can, however, not be said for their combinatorial properties.
Those heavily depend on the studied correctness property.
Memory safety CTs are fairly easy to combine, because memory safety is essentially a local property, as long as we do not change the memory layout relevant for the CT.
We are planning to look into more correctness properties and see whether we can from that extract a locality requirement that allows for CT combinators similar to the memory safety ones.














%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/curriculum/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:04 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: curriculum.pdf
curriculum.pdf: 
	( cd "$(MAINDIR)" && make chapters/curriculum/$@ )

.PHONY: bare curriculum_bare.pdf
bare: curriculum_bare.pdf
curriculum_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/curriculum/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/curriculum/curriculum.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard curriculum*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) curriculum.pdf curriculum_bare.pdf

s:
	@echo gvim curriculum.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/curriculum/curriculum.tex <==
% !TeX root = ../../thesis.tex
\chapter{This is curriculum}\label{ch:curriculum}

\ldots

\instructionscv


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/intro-template-backup/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:05 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: intro-template-backup.pdf
intro-template-backup.pdf: 
	( cd "$(MAINDIR)" && make chapters/intro-template-backup/$@ )

.PHONY: bare intro-template-backup_bare.pdf
bare: intro-template-backup_bare.pdf
intro-template-backup_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/intro-template-backup/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/intro-template-backup/intro-template-backup.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard intro-template-backup*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) intro-template-backup.pdf intro-template-backup_bare.pdf

s:
	@echo gvim intro-template-backup.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/introduction/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:04 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: introduction.pdf
introduction.pdf: 
	( cd "$(MAINDIR)" && make chapters/introduction/$@ )

.PHONY: bare introduction_bare.pdf
bare: introduction_bare.pdf
introduction_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/introduction/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/introduction/introduction.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard introduction*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) introduction.pdf introduction_bare.pdf

s:
	@echo gvim introduction.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/manual/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:04 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: manual.pdf
manual.pdf: 
	( cd "$(MAINDIR)" && make chapters/manual/$@ )

.PHONY: bare manual_bare.pdf
bare: manual_bare.pdf
manual_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/manual/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/manual/manual.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard manual*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) manual.pdf manual_bare.pdf

s:
	@echo gvim manual.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/manual/manual.tex <==
% !TeX root = ../../thesis.tex
\chapter{Manual}\label{ch:manual}


\section{Tips and Tricks}

\subsection{Image on the cover page}

If you want to place an image on the cover of the dissertation, you can add
the code underneath to the template (check with your promotor whether this is
allowed).

\paragraph{Include image:}
Search for the \texttt{\textbackslash frontcoverheaderXII} command in
the \texttt{adsphd.cls} file and add the following lines:
\begin{verbatim}
   \begin{textblock*}{56mm}(10mm+#1,15mm)
   \includegraphics[width=56mm,height=20mm]{image/filename}
   \end{textblock*}
\end{verbatim}
Where 56mm is the width, 20mm the height, 10mm the x-location and 15mm the
y-location.

\paragraph{Change cover font color:}
Add the command \texttt{\textbackslash color\{red\}} to the
\texttt{\textbackslash frontcoverheaderXII} command or enclose specific parts.
For example, \texttt{\{\textbackslash color\{red\}\textbackslash
textbf\{\textbackslash @authorf\textbackslash\ \textbackslash @authorl\}}.

\subsection{Full cover page}

\textbf{Important}: most printing services will create their own cover page based
on the details you send them (title, name, affiliation, ...) and do not supply
you with all necessary parameters (e.g., thickness of the paper) because these
differ from machine to machine. Therefore, the generated cover page is only
indicative and probably not used by your printing server (or even correct).


A full cover page (combining front cover, spine and back cover) can be
generated automatically using the command \texttt{make cover} or \texttt{python3 run.py cover}. This creates a pdf
\texttt{\$(COVERPDF);} by default this is \texttt{cover.pdf}.

The width of the spine is set by redefining \texttt{\\adsphdspinewidth} (9mm by default).

It can be seen in the provided \texttt{thesis.tex} that all information necessary to
generate a cover page is contained between two markers

\begin{verbatim}
    %%% COVER: Settings %%%
    ...
    %%% COVER: End settings %%%
\end{verbatim}

DO NOT REMOVE THESE!! They are used by the Makefile!!

The default front and/or back cover page can be overwritten: 

\begin{itemize}
    \item create a file \texttt{mycoverpage.tex}
    \item redefine the commands \texttt{\textbackslash makefrontcovergeneral} and \texttt{\textbackslash makebackcovergeneral}. For
          an example and more information, see the provided file \texttt{mycoverpage.tex}.
\end{itemize}

The cover page in the generated pdf has the following structure:

{\tiny
\begin{verbatim}
    <--rbleed--><--backcoverpage--><--lbleed--><--spine width--><--lbleed--><--frontcoverpage--><--rbleed-->
\end{verbatim}
}

The default bleed (both lbleed and rbleed) is 7mm. I suggest not changing this
value unless you know what you are doing ;) The latter can be done by
redefining \texttt{\textbackslash defaultlbleed} and \texttt{\textbackslash defaultrbleed} respectively.


\subsection{Table of contents}

To remove list of figures, tables and other preface chapters from the table of
contents, search for occurrences of \texttt{\textbackslash addcontentsline} in the file
\texttt{adsphd.cls} and comment them.

\subsection{Small ebook size}

When you add the \texttt{epub} option to the adsphd class the dissertation is
printed to a smaller size to read on a device such as Kindle.

Environments such as tables or tikZ pictures are often sized in absolute values
and not relative to the size of the output. You can wrap them in a resizebox
to enforce scaling:

\begin{verbatim}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{cc}
      ...
    \end{tabular}
  }
\end{verbatim}

\section{Settings for TeXstudio}

If you are working with TeXstudio or other windows latex editors you might want to adjust the editor's settings to allow a proper compilation of the table of contents and list of figures/tables.

\subsection{Custom \textit{makeindex} and \textit{makeglossaries} commands}

According to the \textit{README.md} the tables are indexed through two custom commands. To edit them in TeXstudio open the \textit{Commands} settings (\textit{Options $\to$ Configure TeXstudio...,  Commands} sheet), edit the following fields and press OK.

\textit{Makeindex}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.nlo -s nomencl.ist -o %.nls
\end{verbatim}}

\textit{Makeglossaries}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.glo -s %.ist -t %.glg -o %.gls
\end{verbatim}}

Now the customized commands can be launched by using \textit{Tools $\to$ Commands $\to$ MakeIndex/Makeglossaries}. If you want to automatize it in the standard \textit{Build \& View} (F5) and \textit{Compile} (F6) commands look at the following section.

\subsection{Custom Build\&View and Compile meta-commands}

Open \textit{Options $\to$ Configure TeXstudio...,  Build} sheet, edit the following field and press OK.

\textit{Build \& View}:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex
	\end{verbatim}}

To view the PDF once created you have to press F7 (or \textit{Tool $\to$ View}) and the PDF will automatically update in the default viewer whan you modify it. 

If you prefer to directly view the created PDF\textbf{ from the beginning }edit the field as follow:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex | txs:///view-pdf
	\end{verbatim}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage



==> chapters/paper-1-abruptExit/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:04 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: paper-1-abruptExit.pdf
paper-1-abruptExit.pdf: 
	( cd "$(MAINDIR)" && make chapters/paper-1-abruptExit/$@ )

.PHONY: bare paper-1-abruptExit_bare.pdf
bare: paper-1-abruptExit_bare.pdf
paper-1-abruptExit_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/paper-1-abruptExit/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/paper-1-abruptExit/paper-1-abruptExit.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard paper-1-abruptExit*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) paper-1-abruptExit.pdf paper-1-abruptExit_bare.pdf

s:
	@echo gvim paper-1-abruptExit.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/paper-1-abruptExit/paper-1-abruptExit.tex <==
% !TeX root = ../../thesis.tex
\chapter{A Separation Logic to Verify Termination of Busy Waiting for Abrupt Program Exit}\label{ch:paper-1-abruptExit}


\TodoTextNote{Delete this section. Content subsumed by Ghost Signal section.}

\NewDocumentCommand{\aeSecDir}{}
	{chapters/paper-1-abruptExit/FTfJP_paper}

This chapter was previously published as:
\citationBox
{
	\textbf{T. Reinhard}, A. Timany, and B. Jacobs. 
	\emph{A Separation Logic to Verify Termination of Busy Waiting for Abrupt Program Exit.}
	In Proceedings of the 22nd ACM SIGPLAN
	International Workshop on Formal Techniques for Java-Like Programs (FTfJP) (2020),
	ACM, pp. 26–32
}



\subfile{\aeSecDir/AbruptExit}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/paper-2-ghostSignals/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:05 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: paper-2-ghostSignals.pdf
paper-2-ghostSignals.pdf: 
	( cd "$(MAINDIR)" && make chapters/paper-2-ghostSignals/$@ )

.PHONY: bare paper-2-ghostSignals_bare.pdf
bare: paper-2-ghostSignals_bare.pdf
paper-2-ghostSignals_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/paper-2-ghostSignals/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/paper-2-ghostSignals/paper-2-ghostSignals.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard paper-2-ghostSignals*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) paper-2-ghostSignals.pdf paper-2-ghostSignals_bare.pdf

s:
	@echo gvim paper-2-ghostSignals.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/paper-3-ct4ms/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:05 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: paper-3-ct4ms.pdf
paper-3-ct4ms.pdf: 
	( cd "$(MAINDIR)" && make chapters/paper-3-ct4ms/$@ )

.PHONY: bare paper-3-ct4ms_bare.pdf
bare: paper-3-ct4ms_bare.pdf
paper-3-ct4ms_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/paper-3-ct4ms/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/paper-3-ct4ms/paper-3-ct4ms.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard paper-3-ct4ms*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) paper-3-ct4ms.pdf paper-3-ct4ms_bare.pdf

s:
	@echo gvim paper-3-ct4ms.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/preface/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:04 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: preface.pdf
preface.pdf: 
	( cd "$(MAINDIR)" && make chapters/preface/$@ )

.PHONY: bare preface_bare.pdf
bare: preface_bare.pdf
preface_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/preface/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/preface/preface.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard preface*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) preface.pdf preface_bare.pdf

s:
	@echo gvim preface.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/preface/preface.tex <==
% !TeX root = ../../thesis.tex
\chapter*{Preface}                                  \label{ch:preface}



I am grateful to my advisor, Bart Jacobs, and my co-advisor, Amin Timany, for providing me with the opportunity to delve further into the realm of software verification and, especially, for introducing me to separation logic.
Your steadfast encouragement and profound expertise have been deeply appreciated, along with all the insightful and interesting discussions we've had.
The insights I gained from separation logic have significantly enhanced my understanding of software verification, an experience I deeply value.
Furthermore, I appreciate the freedom Bart offered me to cultivate and pursue my own visions while venturing into new and uncharted territories.

I want to express my gratitude to my dissertation committee, Marieke Huisman, Peter Müller, Frank Piessens, and Tom Schrijvers, for their insightful evaluation of my dissertation.
Your expertise was invaluable, and I sincerely appreciate the time and effort you dedicated to reviewing my work.
Additionally, I thoroughly enjoyed the engaging and enriching discussion of my thesis during the defence.
I would also like to thank Dirk Vandermeulen for chairing my dissertation committee.

Besides my work in academia, I had the invaluable opportunity to intern twice at Amazon's Automated Reasoning Group.
This experience profoundly impacted not only my personal growth but also my development as a researcher.
I want to extend my heartfelt thanks to my mentor, Nathan Chong, and manager, Mark Tuttle, for the engaging discussions and for their thoughtfulness that defined my time in Boston.
Additionally, I am grateful to my other managers and colleagues, Mike Whalen, Jim Grundy, Saswat Padhi, Felipe Monteiro, Daniel Kroening, and Michael Tautschnig, for our fruitful collaboration.

I want to thank my friend and collaborator Joachim Kristensen for the joint project we recently started.
Working with you has been a pleasure and I am sure that we have some exciting times ahead of us.
I am particularly excited about the opportunity to visit you and your group in Oslo soon.
Next, I want to thank all the people who read my works and listened to my pitches numerous times.
Note that all the feedback you gave me over the years and all the discussions we had are truly appreciated.
While this list is not exhaustive, I want to give particular shout-outs to the following friends:
Friedrich Weber for being my go-to model checking expert and for pointing me to the first work on completeness thresholds I ever read.
Ramana Nagasamudram for your warm and constructive attitude, especially during those discussions that made me change my mind.
Justus Fasse for being the personification of a related work library and for the fun I had during our collaborations.
Next, I want to extend my gratitude to my SIGPLAN mentor Stavros Aronis.
Thanks for sharing your experience with me and for the insightful perspectives you offered during our meetings.

I am happy to say that, during my time in Leuven, I found the most supportive and inclusive circle of friends and fellow PhD candidates one could wish for (in order of first appearance):
Justus Fasse, Nima Rahimi Foroushaani, 
{\DJ}or{\dj}e Markovi\'c, Vida Ranjbar, Niels Mommen, Denis Carnier, Weihong Wang.
All of you are truly amazing and have made my experience in Leuven unforgettable.
Thank you for your unconditional support and the kindness you showed me during the years.
Your friendship has enriched my life in ways I'll always cherish and never forget.

Moreover, I thank my other friends and colleagues in the research community and the department:
Hanneli Tavante, Robbe Van den Eede, Federico Quin, Gints Engelen, Fritz Alder, Shirin Kalantari, Pieter Luyten, Gerald Budigiri, Lesly-Ann Daniel, Ignace Bossuyt, Petra Asma, Katrien Janssens, Annick Vandijck, and An Makowski.

I am deeply thankful to my parents, Erwin and Karin, and my brother, Dominik Reinhard, for their unwavering support and enduring belief in my capabilities.
Their steadfast encouragement has been invaluable, and their continuous support has played a crucial role in helping me pursue and achieve my goals throughout my journey.

Coming to an end, I just want to give a big shout-out to my partner, Carina.
Your support over the years has been nothing short of incredible.
Thank you for always being there to listen to my possibly overly detailed descriptions of random verification topics.
Anyways, without you, none of this would have been possible!
And now, I can't wait to see what adventures await us in the next chapter of our journey together!
Schau'n mer mal was wird.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/publications/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:37:04 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: publications.pdf
publications.pdf: 
	( cd "$(MAINDIR)" && make chapters/publications/$@ )

.PHONY: bare publications_bare.pdf
bare: publications_bare.pdf
publications_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/publications/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/publications/publications.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard publications*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) publications.pdf publications_bare.pdf

s:
	@echo gvim publications.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/publications/publications.tex <==
% !TeX root = ../../thesis.tex
\chapter{List of Contributions}\label{ch:publications}


\paragraph{Published Papers}
\begin{itemize}
	% CTs
	% ------------------------------------------------------------------------------------
	%\item \cite{Reinhard2023ct4ms_atrav_forPubList}
	\item \textbf{T. Reinhard}, J. Fasse, and B. Jacobs. 
				\emph{Completeness Thresholds for Memory Safety of Array Traversing Programs}. 
				In Proceedings of the 12th ACM SIGPLAN 
				International Workshop on the State of the Art in Program Analysis (SOAP) (2023), 
				ACM, pp. 47–54.
				\href
					{https://doi.org/10.1145/3589250.3596143}
					{doi.org/10.1145/3589250.3596143}

	
	
	% Ghost Signals
	% -------------
	%\item \cite{Reinhard2021GhostSignals_forPubList}
	\item \textbf{T. Reinhard}, and B. Jacobs. 
				\emph{Ghost Signals: Verifying Termination of Busy Waiting}.
				In Proceedings of 33rd 
				International Conference on Computer-Aided Verification (CAV) (2021), 
				vol. 12760 of Lecture Notes in Computer Science, Springer, pp. 27–50.
				\\
				\href
					{https://doi.org/10.1007/978-3-030-81688-9_2}
					{doi.org/10.1007/978-3-030-81688-9\_2}
				
				

	% Abrupt Exit
	% -----------
	%\item \cite{Reinhard2020AbruptExit_forPubList}
	\item \textbf{T. Reinhard}, A. Timany, and B. Jacobs. 
				\emph{A Separation Logic to Verify Termination of Busy Waiting for Abrupt Program Exit}.
				In Proceedings of the 22nd ACM SIGPLAN
				International Workshop on Formal Techniques for Java-Like Programs (FTfJP) (2020),
				ACM, pp.~26–32.
				\href
					{https://doi.org/10.1145/3427761.3428345}
					{doi.org/10.1145/3427761.3428345}
	
	
	% Static Latency Tracking
	% Short Paper
	% ---------------------------------------------------------------------------
	\item P. Weisenburger, \textbf{T. Reinhard}, G. Salvaneschi.
				\emph{Static Latency Tracking with Placement Types}.
				In Companion Proceedings for the ISSTA/ECOOP 2018 Workshops.
				(2018)
				ACM, pp.~34–36.
				\\
				\href
					{https://doi.org/10.1145/3236454.3236486}
					{doi.org/10.1145/3236454.3236486}
	
\end{itemize}



\newpage
\paragraph{Posters and Competition Contributions}
\begin{itemize}
	\item \textbf{T. Reinhard}, J. Fasse, and B. Jacobs.
				\emph{Completeness Thresholds for Memory Safety: Unbounded Guarantees Via Bounded Proofs}.
				ACM SIGPLAN International Conference on Systems, Programming, Languages and Applications: Software for Humanity (SPLASH) (2023), 
				Poster Track.
				\href
				{http://doi.org/10.5281/zenodo.10066197}
				{Zenodo doi.org/10.5281/zenodo.10066197}
				
				
	\item \textbf{T. Reinhard}.
				\emph{A Core Calculus for Static Latency Tracking with Placement Types}.
				ACM SIGPLAN Student Research Competition at
				Symposium on Principles of Programming Languages
				(SRC@POPL)
				(2019),
				Extended~Abstract~Round.
				\href
					{https://doi.org/10.48550/arXiv.2007.15617}
					{doi.org/10.48550/arXiv.2007.15617}
	
	\item \textbf{T. Reinhard}.
				\emph{Type-Level Latency Tracking with Placement Types}.
				ACM SIGPLAN Student Research Competition at
				Symposium on Principles of Programming Languages
				(SRC@POPL)
				(2019),
				Poster~Round.
				\href
					{https://doi.org/10.5281/zenodo.10160638}
					{doi.org/10.5281/zenodo.10160638}
				
				
				
\end{itemize}



\paragraph{Abstracts and Technical Reports}
\begin{itemize}
	\item \textbf{T. Reinhard}, J. Fasse, and B. Jacobs.
				\emph{Completeness Thresholds for Memory Safety: Unbounded Guarantees via Bounded Proofs (Extended Abstract)}. 
%				CoRR abs/2309.09731,
				(2023)
				\href
					{https://arxiv.org/abs/2309.09731}
					{arxiv.org/abs/2309.09731}
	\item \textbf{T. Reinhard}.
				\emph{Completeness Thresholds for Memory Safety of Array Traversing Programs: Early Technical Report}.
				(2023)
				\\
				\href
					{https://arxiv.org/abs/2211.11885}
					{arxiv.org/abs/2211.11885}
	\item \textbf{T. Reinhard} and  B. Jacobs.
				\emph{Ghost Signals: Verifying Termination of Busy Waiting (Technical Report)}.
				Zenodo.
				(2021)
				\\
				\href
					{https://doi.org/10.5281/zenodo.4775181}
					{doi.org/10.5281/zenodo.4775181}
	\item \textbf{T. Reinhard} and  B. Jacobs.
				\emph{A Separation Logic to Verify Termination of Busy-Waiting for Abrupt Program Exit: Technical Report}.
				(2020)
				\href
					{https://arxiv.org/abs/2007.10215}
					{arxiv.org/abs/2007.10215}
\end{itemize}



\newpage
\paragraph{Invited Talks}
\begin{itemize}
	\item \emph{Completeness Thresholds for Memory Safety:\@ Unbounded Guarantees Via Bounded Proofs}.
				Programming Languages and Verification Seminar, Portland State University,
				2023
	\item \emph{Completeness Thresholds for Memory Safety:\@ Unbounded Guarantees Via Bounded Proofs}.
				Programming Group, University of St.\@ Gallen (HSG), 
				2023
\end{itemize}

\paragraph{Research Internships}
\begin{itemize}
	\item \!\href
				{https://github.com/Tobias-internship-AWS-2022/FreeRTOS-Kernel/tree/verifast_switch_context/Test/VeriFast/tasks/vTaskSwitchContext}
				{\emph{Verification of the Multicore Implementation of the FreeRTOS Scheduler}}.
			\\
			Low-level Code Reasoning Team, Automated Reasoning Group,\\
			Amazon Web Services (2022)
	\item \emph{Strategies to Progress From Bounded to Unbounded Verification}.\\
			Proof Platforms Team, Automated Reasoning Group,\\
			Amazon Web Services (2021)
\end{itemize}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/state-of-the-art/Makefile <==
# Autogenerated Makefile, Mon Oct  9 16:38:07 CEST 2023.

MAINDIR = /Users/tobias/research/PhD-Thesis/thesis-tex

.PHONY: state-of-the-art.pdf
state-of-the-art.pdf: 
	( cd "$(MAINDIR)" && make chapters/state-of-the-art/$@ )

.PHONY: bare state-of-the-art_bare.pdf
bare: state-of-the-art_bare.pdf
state-of-the-art_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/state-of-the-art/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /Users/tobias/research/PhD-Thesis/thesis-tex/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/state-of-the-art/state-of-the-art.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard state-of-the-art*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) state-of-the-art.pdf state-of-the-art_bare.pdf

s:
	@echo gvim state-of-the-art.tex allpapers.bib > $@
	@chmod +x $@
	@echo You can now start using ./s


==> mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneral{xskip}{clearpage}
%   \makebackcovergeneral{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
\makeatletter

%% \renewcommand{\makefrontcovergeneral}[2]{%
%%   %
%%   % Create header
%%   \frontcoverheader{#1}
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Title, subtitle, authorname, text and date can be moved around.
%%   % Change the textblock* commands below. 
%%   %
%%   % Syntax of textblock environment:
%%   % 
%%   %   \begin{textblock*}{width}(xpos,ypos)
%%   %     ...
%%   %   \end{textblock*}
%%   % 
%%   % !! Make sure not to remove the '+#1' part!!!
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Place the title
%%   \begin{textblock*}{120mm}(17.5mm+#1,89.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \raggedright\selectfont\LARGE\sffamily\textbf{\@title}
%%   \end{textblock*}
%%   %
%%   % Place the subtitle
%%   \begin{textblock*}{120mm}(17.5mm+#1,92.0mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily{\@subtitle}
%%   \end{textblock*}
%%   %
%%   % Place the author name
%%   \begin{textblock*}{120mm}(17.5mm+#1,109.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily\@authorf\ \MakeUppercase\@authorl
%%   \end{textblock*}
%%   %
%%   %\begin{textblock}{120}(0,115)
%%   \begin{textblock*}{120mm}(17.5mm+#1,132.0mm)
%%   \textblockcolour{}
%%   \includegraphics*{image/coverfigure}
%%   \end{textblock*}
%%   %
%%   % Place the misc text
%%   \begin{textblock*}{60mm}(96.5mm+#1,187.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   {\small\sffamily Dissertation presented in partial\\
%%   fulfillment of the requirements for\\
%%   the degree of Doctor\\
%%   in \@degree}
%%   \end{textblock*}
%%   %
%%   % Place date
%%   \begin{textblock*}{160mm}(0mm+#1,221.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \begin{center} {\small\sffamily\@date }\end{center}
%%   \end{textblock*}
%%   
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Add footer
%%   \frontcoverfooter{#2}
%% 
%% }

\makeatother

